Prompt Perturbation Consistency Learning for Robust Language Models

Large language models (LLMs) have demonstrated impressive performance on a number of natural language processing tasks, such as question answering and text summarization. However, their performance on sequence labeling tasks such as intent classification and slot filling (IC-SF), which is a central component in personal assistant systems, lags significantly behind discriminative models. Furthermore, there is a lack of substantive research on the robustness of LLMs to various perturbations in the input prompts. The contributions of this paper are three-fold. First, we show that fine-tuning sufficiently large LLMs can produce IC-SF performance comparable to discriminative models. Next, we systematically analyze the performance deterioration of those fine-tuned models due to three distinct yet relevant types of input perturbations - oronyms, synonyms, and paraphrasing. Finally, we propose an efficient mitigation approach, Prompt Perturbation Consistency Learning (PPCL), which works by regularizing the divergence between losses from clean and perturbed samples. Our experiments demonstrate that PPCL can recover on average 59% and 69% of the performance drop for IC and SF tasks, respectively. Furthermore, PPCL beats the data augmentation approach while using ten times fewer augmented data samples.

==> abstract.tex <==
\begin{abstract}
Large language models (LLMs) have demonstrated impressive  performance on a number of natural language processing tasks, such as question answering and text summarization. However, their performance on sequence labeling tasks such as intent classification  and slot filling (IC-SF), which is a central component in personal assistant systems, lags significantly behind discriminative models. Furthermore, there is a lack of substantive research on robustness of LLMs to various perturbations in the input prompts. The contributions of this paper are three-fold. First, we show that fine-tuning sufficiently large LLMs can produce IC-SF performance comparable to discriminative models. Next, we systematically analyze the  performance deterioration of those fine-tuned models due to three distinct yet relevant types of input perturbations - oronyms, synonyms, and paraphrasing. Finally, we propose an efficient mitigation approach, {\em prompt perturbation consistency learning} (PPCL), which works by regularizing the divergence between losses from clean and perturbed samples. Our experiments demonstrate that PPCL can recover on an average 59\% and 69\% of the performance drop for IC and SF tasks, respectively. Furthermore, PPCL beats data augmentation approach while using ten times fewer augmented data samples.
%Pre-trained generative large language models (G-LLMs) when fine-tuned on high quality data have demonstrated SOTA performance in different NLP tasks. However, their performance on sequence labeling tasks such as intent classification (IC) and slot filling (SF) still lag behind discriminative LLMs (D-LLMs). Recent studies have shown G-LLMs to be sensitive to automatic speech recognition (ASR) errors or oronyms. There is a lack of substantive research on robustness of fine-tuned G-LLMs to prompt perturbations other than oronyms, such as synonyms and semantically similar paraphrasing in the prompts. Our contribution is two-fold. First we show that fine-tuning some of the larger G-LLMs can produce IC-SF performance comparable to D-LLMs. Next, we quantify the drop in performance with the three prompt perturbations. Self-augmentation is a widely used approach to increase LLM robustness. However, that comes at the cost of ballooning training data size. We propose an efficient prompt perturbation consistency learning (PPCL) by regularizing the divergence between losses from clean and perturbed samples. We show that PPCL can recover on an average 60\% of the performance drops in IC tasks and 69\% in SF tasks. PPCL beats data augmentation approach with only 10\% of augmentation size.
\end{abstract}

==> conclusion.tex <==
\section{Conclusion}
\noindent
We study, evaluate, and improve the robustness of LLMs in generating structured hypotheses, such as IC-SF tasks in this work. We first propose a sentinel-based structured prompt format for instruction fine-tuning LLMs resulting in comparable performance to SOTA discriminative models. Furthermore, we evaluate the robustness of LLMs under various prompt perturbations, i.e., synonyms, oronyms, and paraphrases. Our results indicate that LLMs are vulnerable to these perturbations, with an average performance drop rate of 13.07\% in IC accuracy and 22.20\% in SF F1-score. We then propose two mitigation strategies, i.e., perturbation consistency learning and data augmentation, aiming to improve model robustness. These methods are able to recover up to 59\% performance drop in IC task and 69\% in SF task, making the resulting LLMs more robust to prompt perturbations.

==> experiment.tex <==
\section{Experiments}
\subsection{Experimental Settings}
\noindent
\paragraph{Datasets}
We evaluate model performance on three NLU benchmark datasets, i.e., ATIS \cite{price1990evaluation}, SNIPS \cite{coucke2018snips}, MASSIVE \cite{fitzgerald2022massive}. More details of these datasets and their statistics are shown in the Appendix. 

\paragraph{Baselines} 
We compare the performance of PPCL with the following baselines: supervised fine-tuning with discriminative models like JointBERT and JointBERT+CRF, zero-shot and few-shot learning with GPT variants, instruction fine-tuning with LLaMA. For additional information about these baselines and their specific experimental setups, please refer to the Appendix.

\subsection{Evaluation Metrics}
\noindent
For IC task, we use prediction accuracy on a held out testset and for SF task we use F1-score as  the evaluation metrics.


Instead of using absolute difference in performance between models trained with clean and and perturbed data, we use a relative measurement. We introduce Performance Drop Rate (PDR), which quantifies the relative performance decline following a perturbation, formally: 
\begin{equation}
    \mathrm{PDR}(\mathcal{D},\mathcal{D}^\prime,f_\theta) = 1 - \frac {\sum_{(x,y)\in{\mathcal{D^\prime}}}\mathcal{M}[f_\theta(x),y]}{\sum_{(x,y)\in{\mathcal{D}}}
\mathcal{M}[f_\theta(x),y]}.
\end{equation}
$\mathcal{M}$ here is the indicator function and $f_\theta$ denotes the models. $\mathcal{D}$ and $\mathcal{D}^\prime$ indicates the clean and perturbed test sets, respectively. We want to clarify that the clean and perturbed test sets have a one-to-one corresponding relationship, thus $|\mathcal{D}| == |\mathcal{D}^\prime|$. In other words, each example in the clean test set has a corresponding example in the perturbed test set. This ensures a fair and direct comparison between the model's performance on clean and perturbed samples.

\subsection{Perturbed Evaluation Sets}
\noindent
We generate perturbed evaluation sets for each benchmark dataset. For IC-SF tasks we compile a list of key stop words based on the domain, intent, and slot label sets, and do not substitute them. To ensure that clean and perturbed samples are semantically similar, we filter out perturbations with BERTScore \cite{zhang2019bertscore} with the original sample. We use a 0.85 threshold.

With perturbations of samples, generating appropriate target labels is crucial for evaluation. For intent labels, we align them with those of the original utterances. For slot labels, the procedure is more complex. For perturbations that maintain the length and word order, such as oronyms and synonyms, we directly adopt the original slot labels as their corresponding counterparts. For paraphrased variations that may deviate in length and word order from the original utterance, we automatically generate new slot labels. The new slot labels are derived from the semantic annotations present in the original utterance. This strategy ensures that the perturbed versions retain their intended meaning while accommodating any structural changes arising from the paraphrasing process.

==> introduction.tex <==
\section{Introduction}
\noindent
Voice controlled smart personal assistants like Amazon Echo and Google Home have flourished in recent years, enabling goal-oriented conversations and aiding tasks like setting reminders, checking weather, controlling smart devices, and online shopping. A crucial aspect of their effectiveness lies in their ability to understand user requests (e.g., setting reminders, fetching weather information, etc.) and respond or act appropriately to meet particular requirements. The majority of these applications heavily depend on voice interactions, making it imperative to have a strong grasp of spoken language understanding (SLU) \cite{young2013pomdp}. SLU usually commences with automatic speech recognition (ASR), which involves converting spoken language into written text. Following ASR are natural language understanding (NLU) tasks, such as question answering, dialogue management, intent classification (IC), and slot filling (SF) \cite{tur2011spoken,qin2021survey}. In particular, the IC task involves identifying the speaker's desired intent from a given utterance, while slot filling (SF) involves recognizing the key arguments of the intent. To illustrate, consider the user query: ``wake me up at five am this week.", the intent is `set alarm'. Meanwhile, the SF component should identify the specific details, such as `five am' as time and `this week' as date for the alarm setting. By combining these two tasks, the assistants can accurately understand the user's request and take appropriate actions accordingly. 

Pre-trained large language models (LLMs) hold promise of greatly improving personal assistant systems, owing to their impressive conversational and reasoning capabilities. In addition to generating fluent conversations, LLMs have shown SOTA performance on a variety of natural language processing (NLP) tasks  such as text classification, question answering, text summarization~\cite{brown2020language,chowdhery2022palm,qin2023chatgpt}. Furthermore, some LLMs have shown promising ability to generate structured outputs such as code synthesis~\cite{nijkamp2023codegen2,li2023starcoder} and API calls~\cite{patil2023gorilla}. However, the performance of LLMs on other structured prediction tasks such as slot filling lags significantly behind supervised baselines \cite{srinivasan2023multilingual}. 

Another important issue is that LLMs can be highly sensitive to prompt variations~\cite{webson-pavlick-2022-prompt,min-etal-2022-rethinking,ye2022the}. For instance, varying  the order of few-shot examples, introducing minor typos or different expressions with the same semantic meaning can lead to qualitatively different results~\cite{jin2020bert,li2020bert,huang2021robustness,zhuo2023robustness}. In conversational systems, such perturbations might be caused by  ASR errors, linguistic differences, and user-specific expressions. Thus, adopting LLMs for voice-based personal assistant systems requires a good understanding of their robustness  to above types of perturbations, and effective mitigation strategies for ensuring robustness of LLMs based IC-SF models.   


%The main reason for this performance gap lies in the inherent differences between SF and LLMs. SF involves assigning entity-type labels to each token within an utterance, making it a sequence labeling task. On the other hand, LLMs are designed for text generation tasks. The mismatch between the nature of the semantic labeling task and the design of text generation models results in lower performance when LLMs are used to tackle the SF task.


%In addition to the performance gap, the robustness of LLMs on IC-SF tasks is another issue that has not been thoroughly studied. LLMs are known to be highly sensitive to prompt perturbations, e.g., the order of few-shot examples, minor typos, or different expressions with the same semantic meaning, can lead to qualitatively different results \cite{jin2020bert,li2020bert,huang2021robustness,zhuo2023robustness}. Real world data often contains variations caused by ASR errors, linguistic differences, and user-specific expressions. Addressing robustness to noisy data remains a critical research area in NLP to ensure the practical applicability of IC-SF models in real-world scenarios. Nevertheless, the relentless improvement of pre-trained LLMS across diverse tasks is leading to their increasing adoption in most NLP applications. For safety-critical and decision-making domains, it is essential to understand the robustness of these methods and how it can be improved. 

\begin{figure*}[t]
  \centering 
  \includegraphics[width=0.98\textwidth]{illustration.pdf}
  \caption{Illustration examples. LLMs are expected to generate structured hypotheses, i.e., domain, intent, and slots, in their responses to given user requests.}
  \label{fig:illustration} 
\end{figure*}

In this paper we consider the following questions:
\begin{enumerate}
    \item How can we close the performance gap between LLMs and SOTA discriminative models on IC-SF tasks?
    \item How does the performance of LLMs change with small changes to the original utterances?
    \item Can we improve robustness of LLMs in the cases of  realistic perturbations?
\end{enumerate}
%By investigating and answering these questions, we aim to provide valuable insights into the reliability and effectiveness of prompt-based approaches in handling perturbed or noisy data, which is crucial in real-world NLP applications. 

To address the first question, we explore supervised  fine-tuning (SFT) for the IC-SF task, where the base LLM is asked to generate a target output based on an input query. We conduct extensive experiments on three publicly available NLU benchmark datasets (ATIS, SNIP, MASSIVE) and show that by combining prompt selection and SFT on moderately sized datasets, LLMs can learn to generate structured IC-SF hypotheses with accuracy that is on par with SOTA discriminative method.  

Next, we systematically explore the robustness of the fine-tuned models to three different types of input perturbations that are relevant in the context of voice assistant systems -- oronyms, synonyms, and paraphrasing. These types of perturbations are omnipresent in real world data  due to  ASR errors, linguistic differences, and user-specific expressions. We observe that all three types of  perturbations  negatively impact the model performance, with the performance drop most significant for the SF task when the inputs are subject to oronym perturbations.

Finally, we explore methods for obtaining robust LLM-based IC-SF  models against such perturbations. The most common approach for obtaining robust models followed by past NLP research has been via adversarial training \cite{madry2017towards,shafahi2020universal}, which  involves generating and incorporating adversarial examples into the training process to enhance the model's ability to handle perturbations and variations in the input data. While this technique has shown promise for smaller models, applying it to LLMs is computationally intensive and resource-consuming, making it impractical for most real-world applications. Augmenting data by adding variations of the training data can efficiently improve model performance in low-resource scenarios \cite{wei2019eda,zhang2017mixup}, but synthetic samples can potentially alter the semantics of the data in unintended ways. Therefore, alternative methods that strike a balance between robustness, computational efficiency, and semantic uniformity of the augmented samples are essential for ensuring the practical viability of LLMs in handling perturbed data.

Here we propose a novel framework that we call \textit{prompt perturbation consistency learning}, or PPCL, to improve the robustness of LLMs against perturbations. Our framework (1) generates perturbed counterparts given the original utterance by either replacing a small subset of tokens or paraphrasing the utterance while constraining the semantic similarity, (2) fine-tunes LLMs with an additional consistency regularization term in the objective which explicitly encourages the model to generate consistent predictions (and hence consistent response) for the original utterance and its perturbed counterpart. We conduct extensive experiments and demonstrate that PPCL can recover on an average 60\% and 69\% of the dropped performance drops for IC and SF tasks, respectively. Furthermore, our results indicate that PPCL outperforms simple data augmentation approach while using only 10\% of augmented dataset.  




==> method.tex <==
\section{Method}

\subsection{Problem Formulation}
\noindent
Our main objective is to utilize LLMs for the purpose of generating structured hypotheses. As illustrated in Figure \ref{fig:illustration}, LLMs are expected to generate correct, coherent, and structured responses, including domain, intent, and slot labels, based on user utterances. To fill the performance gap between LLMs and SOTA discriminative models, we apply instruction fine-tuning, a well-established fine-tuning method \cite{touvron2023llama}, aiming to enhance their capability to generate the intended structured hypotheses.

We decompose our task into five steps: (1) Prompts Construction: we design several prompt structures, outlined in Appendix Table \ref{tab:prompt}, to be employed during our instruction fine-tuning process. These prompts utilize the input utterances $X$ and the target outputs $Y$, which encompass various labels such as $Y_\mathrm{domain}$, $Y_\mathrm{intent}$, and $Y_\mathrm{slots}$; (2) Instruction Fine-tuning: during instruction fine-tuning, we utilize both the input ($X$) and output ($Y$) within the prompt structure, denoted as Prompt($X,Y$). This approach assists LLMs in learning the task of predicting structured hypotheses, specifically focusing on tasks like IC-SF within our investigation; (3) Response Generation: subsequent to instruction fine-tuning, we employ prompts with only input data, referred to as Prompt($X$), to elicit responses from the LLMs. These responses manifest as a generated text sequence, denoted as $W = \{w_1, \cdots, w_n\}$; (4) Obtaining Structured Hypotheses:  the generated text sequence $W$ is then transformed into structured hypotheses, culminating in the final outcomes denoted as $\{\hat{Y}_\mathrm{domain}, \hat{Y}_\mathrm{intent}, \hat{Y}_\mathrm{slots}\}$; (5) Performance Evaluation: we evaluate the performance by comparing the ground truth labels $\{Y_\mathrm{domain}, Y_\mathrm{intent}, Y_\mathrm{slots}\}$ with the outputs from the LLMs $\{\hat{Y}_\mathrm{domain}, \hat{Y}_\mathrm{intent}, \hat{Y}_\mathrm{slots}\}$. Various metrics are employed for this evaluation, e.g., accuracy and F1-score for IC and SF, respectively.

LLMs exhibit vulnerability to perturbations \cite{zhuo2023robustness,zhu2023promptbench}, leading to the generation of incorrect responses, as demonstrated in Figure \ref{fig:illustration}. By introducing small perturbations to the inputs $X$ or expressing the input differently while preserving the same meaning would result in distinct inputs denoted as $X^\prime$. Nevertheless, given that $X^\prime$ maintains identical structured hypotheses and target labels $Y$, our expectation remains that LLMs should still be able to generate correct responses, thereby yielding the desired outcomes. In other words, LLMs are expected to be robust against these perturbations and generate consistent responses. This highlights the necessity of proposing strategies to mitigate these challenges, thereby enhancing the robustness of LLMs against such perturbations.

\subsection{Prompts Construction}
\noindent
The standard prompts employed during instruction fine-tuning process with LLMs typically involve presenting both the input context and its corresponding target output in a paired structure \cite{liu2023pre}. The LLMs are then trained to generate the target output based on the input context. The primary objective here is to fine-tune the models' parameters aiming to minimize prediction errors and improve their ability to generate accurate and contextually appropriate responses. Therefore, the process of instruction fine-tuning gains advantages not only from an extensive dataset but also from well-structured prompts, particularly when dealing with specific tasks like IC-SF.

We construct several prompt formats for IC-SF tasks as detailed in Appendix Table \ref{tab:prompt}. In more details, the simple prompt format involves presenting the utterance and target outputs consecutively. Additionally, we design a structured prompt format that takes into account the task of predicting structured hypotheses. As exemplified in Appendix Table \ref{tab:prompt}, this format associates the intent with its corresponding domain and aligns the slot labels with the arguments of the request.

Furthermore, in the context of the sequence labeling task, i.e., SF, it is expected that LLMs generate slot labels for each individual token within the given utterance. Effectively associating tokens with their respective slot labels is crucial to enhance the models' performance during instruction fine-tuning. Therefore, we construct three different SF prompt formats with the intention of improving model proficiency in the SF task, as depicted in Appendix Table \ref{tab:prompt}. The tag-only format represents the simplest approach, but it significantly intensifies the learning challenge since the model is required to implicitly track token indices as well \cite{raman2022transforming}. To simplify the tracking of each token in the utterances, we introduce sentinel-based formats. These sentinel markers enable us to avoid redundant inclusion of the original tokens in the target output. Instead, the sentinel tokens are employed to facilitate the learning of associations between tokens and their corresponding slot labels.

Our constructed prompt formats offer several advantages: (1) The structured format efficiently arranges the input and output labels within a coherent structure, facilitating the generation of structured hypotheses; (2) The sentinel-based formats eliminate the need for redundant input repetition, simplifying the decoding process and preventing hallucinations; (3) These formats enable a more straightforward method for token tracking (including indices) and establishing connections between tokens and their corresponding slot labels.

\subsection{Perturbations}
\noindent
A robust model aims to convert all utterances with or without meaning-preserving perturbations into correct hypotheses. To evaluate the model robustness in IC-SF tasks, we employ different types of perturbations, i.e., oronyms, synonyms, and paraphrases, covering both word-level and sentence-level perturbations aligned with real-world application scenarios. We show some examples of these perturbations in Appendix Table \ref{tab:perturbations} and present more details of the generation process in Experiments section.    

Oronym perturbation involves making changes to a text by replacing words or phrases with other words or phrases that are phonetically similar but carry different semantic meanings. Oronym perturbation is widely used for data augmentation in NLP tasks, especially for tasks that require robustness to speech recognition errors (ASR) or homophonic ambiguity \cite{cai2023dialogvcs}. While the altered semantics of oronym-perturbed expressions may differ from the initial utterances, our expectation remains that LLMs can exhibit robustness in the face of these changes and produce responses aligned with user intent.

Synonym perturbation refers to modifications or variations made to a text by replacing certain words or phrases with their synonyms while preserving the overall meaning of the text. It is commonly employed in NLP as data augmentation to enhance data diversity by generating new variations of a given sentence while upholding semantic coherence \cite{alfonso2021nature}. The intention behind utilizing synonym perturbation is to evaluate the robustness of LLMs in generating consistent hypotheses when presented with semantically similar utterances.

Paraphrasing perturbation entails rephrasing a given text to create variations while preserving its original meaning. Paraphrasing perturbations often convey the same basic information as the original texts but use different word choices and structures. This is highly consistent with our daily communications that present the same meaning in different ways. Hence, irrespective of the chosen words or structures, LLMs should consistently produce accurate hypotheses.

\subsection{Data Augmentation}
\noindent
Data augmentation is a valuable strategy in the context of fine-tuning LLMs to improve their performance and generalization capabilities. There are two major benefits of applying data augmentation: (1) It expands the dataset, which proves particularly beneficial for overcoming limited training data in diverse real-world scenarios; (2) It diversifies the fine-tuning dataset, equipping the model to better handle linguistic variations and consequently enhancing its performance in downstream tasks.

In particular, we apply a range of data augmentation techniques, each designed to generate diverse data through specific perturbations. This strategy ultimately contributes to improved model performance, generalization and robustness. To elaborate, we utilize word replacement techniques involving oronyms and synonyms as forms of data augmentation. This approach improves LLMs ability in better adapting to previously unseen data, comprehending language variations, and effectively addressing challenges associated with speech recognition and linguistic ambiguity. Furthermore, considering paraphrasing as the practice of rewording sentences while retaining their original meaning, we propose to generate paraphrased iterations of the training data, providing LLMs with more examples to learn different ways of expressing the same content.

However, even though data augmentation is advantageous, it is essential to strike a balance to prevent the introduction of noise or potentially misleading content. We establish specific constraints during the generation process and implement various post-processing filters to reinforce the preservation of the original utterances' integrity. 

\subsection{Prompt Perturbation Consistency Learning (PPCL)}

\begin{figure*}[t]
  \centering 
  \includegraphics[width=0.75\textwidth]{pcl.pdf} % 
  \caption{Perturbation consistency learning architecture. $x_c$ and $x_p$ denote the clean and perturbed utterances, respectively. $\hat{y}_c$ and $\hat{y}_p$ here denote the slot labels generated by LLM. $\hat{y}_c^j$ and $\hat{y}_p^j$ represent the output probability distributions of current interest tokens, i.e., `date' and `O'. JS here denotes Jensen–Shannon divergence.} 
  \label{fig:pcl} 
\end{figure*}

\noindent
Despite the fact that data augmentation has been demonstrated to be efficient to improve model robustness and generalizability \cite{chen2021hiddencut}, it overlooks the similar semantic meaning shared between the original and augmented data. To address this, we propose a perturbation consistency learning framework to further utilize these augmented data, particularly the perturbed counterparts of the original utterances in our study. The key idea is to integrate a term into the training objective that explicitly encourages the generation of similar predictions (and consequently, comparable responses) for both the original utterance and its perturbed counterpart. Through the incorporation of this additional constraint, our goal is to strengthen the model's ability to maintain consistency between the original and perturbed utterances, resulting in improved robustness and more reliable performance across real-world applications.

More precisely, our objective is to align the model's responses when presented with two semantically equivalent utterances. To achieve this, we incorporate an extra component into the training objective, referred to as the Jensen-Shannon (JS) divergence of output probabilities between a clean utterance and its perturbed counterpart. This term is integrated with the standard cross-entropy loss utilized in the auto-regression phase of the fine-tuning process.

The architecture of PPCL is illustrated in Figure \ref{fig:pcl}. Specifically, during the fine-tuning process, we simultaneously input the clean utterance denoted as $x_c$ and its perturbed counterpart labeled as $x_p$ to the LLMs. In response to these inputs, the LLMs generate corresponding outputs, respectively. We denote $p_c^j$ and $p_p^j$ as the probability distribution over vocabulary of the $j$-th output token for $x_c$ and $x_p$, where $p_c^j,p_p^j \in \mathbb{R}^{|\mathcal{V}|}$ and $\mathcal{V}$ denotes the vocabulary size. Subsequently, we apply Softmax to $p_c^j$ and $p_p^j$ and get their respective probability distributions $\hat{y}_c^j$ and $\hat{y}_p^j$, formally: $\hat{y}_c^j = \mathrm{Softmax}(p_c^j)$ and $\hat{y}_p^j = \mathrm{Softmax}(p_p^j)$.

Subsequently, we apply JS divergence to quantify the similarity between $\hat{y}_c^j$ and $\hat{y}_p^j$. JS is a symmetric variation of Kullback–Leibler divergence (KL), defined as: 
\begin{equation}
    \label{eq:JSD}
    \mathrm{JS}(P||Q) = \frac{1}{2}(\mathrm{KL}(P||M) + \mathrm{KL}(Q||M)), 
\end{equation}
where $M = \frac{1}{2}(P + Q)$. JS smooths out the asymmetry of KL and offers a more balanced perspective on similarity. 
Furthermore, it demonstrates to be more robust since both distributions have areas of extremely low probability, indicating sparsity. Thus, we obtain the JS of the two probability distributions of $j$-th output, denoted as: $\mathrm{JS}(\hat{y}_c^j\ ||\ \hat{y}_p^j)$. We use the average JS across all output probability distributions associated with $x_c$ and $x_p$ as our final perturbation consistency learning loss, formally: 
\begin{equation}
    \label{eq:L_JSD_v1}
    \mathcal{L}_\mathrm{JS} = \frac{1}{L} \sum_{j=1}^L \mathrm{JS}(\hat{y}_c^j\ ||\ \hat{y}_p^j),
\end{equation}
$L$ here denotes the length of the generated response. 

Utilizing Eq. \ref{eq:L_JSD_v1} with oronym and synonym perturbations is straightforward, as these perturbations merely substitute tokens or phrases with their respective oronyms and synonyms while maintaining the utterance length. However, the case of paraphrasing perturbations introduces varying lengths between the clean utterance and its modified counterpart. Instead of computing the JS for each token-pair in the output, we employ the averaged probability distribution to calculate the perturbation consistency learning loss for paraphrasing perturbations, formally:
\begin{equation}
    \label{eq:L_JSD_v2}
    \mathcal{L}_\mathrm{JS} = \mathrm{JS}(\overline{\hat{y}_c}\ ||\ \overline{\hat{y}_p}),
\end{equation}

\subsection{Training Objective}
\noindent
Our training objective integrates the supervised cross-entropy losses for both clean and perturbed utterances (i.e., $\mathcal{L}_C$ and $\mathcal{L}_P$) with the perturbation consistency learning loss $\mathcal{L}_\mathrm{JS}$, formally:
\begin{equation}
   \mathcal{L}_C = \mathrm{CE}(\hat{y}_c, y), 
\end{equation}
\begin{equation}
   \mathcal{L}_P = \mathrm{CE}(\hat{y}_p, y),
\end{equation}
\begin{equation}
   \label{eq:objective}
   \mathcal{L} = \lambda_1 \mathcal{L}_C + \lambda_2 \mathcal{L}_P + \lambda_3 \mathcal{L}_\mathrm{JS},
\end{equation}
where $\lambda_1$, $\lambda_2$, and $\lambda_3$ are weight coefficients.

In order to optimize the above objective, it is essential to have both the clean utterance and its corresponding perturbed counterpart. We generate these paired perturbed utterances using our proposed perturbation generation methods. Furthermore, to ensure the presence of semantically comparable pairs, we implement specific post-processing filtering procedures. These filters serve to verify that the generated perturbed utterances genuinely maintain semantic equivalence with their clean counterparts.

==> relatedwork.tex <==
\section{Related Work}

\paragraph{Intent Classification and Slot Filling} Intent classification focuses on automatically detecting a user's intent from an utterance, which can be treated as a sentence classification problem that predicts the intent category for an utterance. Various techniques have been explored for this task, with recent work focusing on transformer-based models and transfer learning with pre-trained language models~\cite{qin2021survey}. Meanwhile slot filling extracts the relevant semantic concepts from an utterance towards achieving a goal or finishing specific tasks. This task is typically approached using sequence labeling models, such as conditional random fields (CRFs), bidirectional LSTMs, and more recently, transformer-based architectures~\cite{weld2022survey,chen2019bert,goo2018slot} and pre-trained generative LLMs~\cite{he2023can}. Slot filling often requires domain-specific data and involves the challenge of handling out-of-vocabulary (OOV) words. 
Slot filling training data is often expensive to obtain so methods like data augmentation that can help in low-resource scenarios are of particular interest.

\paragraph{Data Augmentation}
Data augmentation is a technique used to increase the amount of training data by creating new and realistic-looking examples without changing the original labels. 
%It is particularly valuable in scenarios where there is a shortage of labeled training data, as it helps improve the performance and generalization of models. 
In NLP tasks, data augmentation methods have been explored to generate new instances by manipulating a few words in the original text~\cite{feng2021survey,chen2023empirical}. Some common techniques include word replacement, where certain words are replaced with synonyms or similar words; random deletion, where words are randomly removed from the text; and word position swap, where the positions of words are shuffled~\cite{wei2019eda}. Additionally, data augmentation in NLP can involve creating entirely artificial examples using back-translation~\cite{sennrich2015improving} or generative models like variational auto-encoders~\cite{malandrakis2019controlled,yoo2019data}. 
%
Data augmentation has also become popular for NER tasks. 
%Researchers have been actively exploring various data augmentation techniques to enhance NER model performance and address data scarcity challenges. 
\citet{dai2020analysis} focused on analyzing the impact of simple data augmentation methods on NER tasks. The study explored techniques like synonym replacement and word swap as forms of data augmentation. In synonym replacement, certain words in the text are replaced with their synonyms or similar words. Word swap involves shuffling the positions of words in the sentences. The success of these and other simple data augmentation techniques in NER tasks highlights the potential of data augmentation as an effective strategy to boost model performance~\cite{meng2021distantly,zhou2021melm}. 
%As the field of NER continues to advance, more sophisticated data augmentation approaches tailored to NER-specific characteristics may be developed, further improving the robustness and accuracy of NER models.

\paragraph{Consistency Training}
Consistency training methods aim to improve the robustness of models by enforcing the stability of their predictions under small perturbations, such as random noise, adversarial noise, or data augmentation techniques, applied to input examples or hidden states. The underlying intuition is that a good model should be able to maintain its accuracy and stability even in the presence of minor changes in the input or hidden representations, reflecting a more reliable and adaptable performance in real-world scenarios. By making the model's predictions consistent despite such perturbations, the framework encourages the model to learn more generalized and smooth output distributions, promoting its overall robustness and ability to handle variations in the input data.

Several attempts have been made to implement consistency training in NER tasks, utilizing both token-level and sequence-level approaches. Token-level consistency involves regularizing the model to remain unaffected by Gaussian noise~\cite{lowell2020unsupervised} or word replacement, operating at the same granularity as NER~\cite{dai2020analysis,liu2022low}. However, using such simplistic noise or augmentation methods may violate the assumption that the noised tokens should retain the same labels as the original tokens. As a result, their performance is limited due to a strong correlation between the perturbation quality and consistency training's effectiveness. Alternatively, a sequence-level consistency method employs high-quality augmentation, like back-translation, to enhance consistency across the entire sentence~\cite{xie2020unsupervised}. Nonetheless, this approach overlooks the precise location of entities due to word alignment issues, leading to a sub-optimal design. More recently, ConNER has been proposed to foster consistent predictions between a span of tokens in the original sentence and their corresponding projection in a translated sentence~\cite{zhou2022conner}. Unfortunately, ConNER's applicability is confined to cross-lingual NER tasks.

Consistency training for fine-tuning LLMs on IC-SF tasks has not been thoroughly explored yet. To address this gap, we introduce a new perturbation consistency learning framework. The goal of this framework is to improve the robustness of LLMs by encouraging them to generate consistent responses either on a token-level or entity-level basis. By enforcing such consistency during fine-tuning, we aim to improve the model's performance and generalization on IC-SF tasks.
\noindent

==> results_discussion.tex <==
\section{Results and Discussion}

\begin{table}[t]
\centering
\small
\caption{Comparison of model performance on three datasets. The best performance of SOTA discriminative models and LLMs is highlighted in bold.$^1$}
\label{tab:baselines}
\begin{tabular}{llcc}
\hline
\textbf{Datasets} & \textbf{Model}\footnotemark & \textbf{Intent Acc} & \textbf{Slot F1} \\
\hline
 & JointBERT & \textbf{89.44} & 80.43 \\
 & JointBERT+CRF & 88.67 & \textbf{80.58} \\
 & GPT3.5-ZS & 60.39 & - \\
MASSIVE & GPT3.5-FS & 67.18 & 31.76 \\
 & GPT2+SFT & 84.13 & 66.72 \\
 & LLaMA-7b+SFT & 88.01 & 80.45 \\
 & LLaMA-13b+SFT & 88.87 & 80.7 \\
 & LLaMA-30b+SFT & \textbf{89.05} & \textbf{80.74} \\
\hline
 & JointBERT & \textbf{97.53} & \textbf{95.83} \\
 & JointBERT+CRF & 96.75 & 95.58 \\
ATIS & GPT3.5-ZS & 87.45 & - \\
 & GPT3.5-FS & 93.17 & 73.51 \\
 & GPT2+SFT & 97.31 & 83.92 \\
 & LLaMA-7b+SFT & \textbf{98.21} & \textbf{94.26} \\
\hline
 & JointBERT & \textbf{98.57} & \textbf{96.67} \\
 & JointBERT+CRF & 98.28 & 96.07 \\
SNIPS & GPT3.5-ZS & 95.14 & - \\
 & GPT3.5-FS & 94.42 & 49.12 \\
 & GPT2+SFT & 97.14 & 88.23 \\
 & LLaMA-7b+SFT & \textbf{98.14} & \textbf{94.51} \\
\hline
\end{tabular}
\footnotetext[1]{CRF: Conditional Random Field; FS: Few Shot; SFT: Supervised Fine Tuned; ZS: Zero Shot}
\vspace{0.25cm}
\end{table}


\subsection{Performance Gap between LLMs and discriminative models}
\noindent
First, we show the model performance comparison of different baselines on three datasets in Table \ref{tab:baselines}. These results demonstrate that LLMs, i.e., GPT2 and LLaMA, which have been instruction fine-tuned with our proposed sentinel-based structured format, achieve comparable intent classification performance to SOTA discriminative models like JointBERT across all three datasets. However, applying zero-shot and few-shot learning settings  the performance of LLMs is notably worse, especially for the SF tasks.

The lower performance of LLMs on the SF task could be attributed to the mismatch between the nature of the semantic labeling task and the design of text generation models. Text generation models like LLMs are not inherently optimized for the SF tasks, which might lead to sub-optimal results in some cases. However they can still achieve comparable results for the sequence labeling task, such as SF, after supervised fine-tuning with appropriate instructions or structured formats. This is demonstrated by LLaMA-30b achieving and average SF accuracy (89.84\%) within 1.3\% of JointBERT performance (91.03\%), and even superseding it for MASSIVE dataset.

\subsection{Prompt Formats}
\noindent
We compare the model performance using different prompt formats in Table \ref{tab:promptformats}. These results demonstrate that the sentinel-based structured prompt format achieves the best performance, particularly for the SF tasks. This outcome aligns with our initial hypothesis that the structured format is highly effective in organizing both the input and output labels, leading to improved learning ability for the models. In addition, sentinel-based slot formatting significantly improves performance, especially in the SF task. 

\begin{table}[h]
\centering
\small
\caption{Comparison of model performance with different prompt formats: Simple and Structured prompt formats with tag-only, extractive sentinel-based with tag, and sentinel-based with tag slots formats, respectively.}
\label{tab:promptformats}
\begin{tabular}{llll}
\hline
\head{1cm}{\textbf{Datasets}} & \head{4cm}{\textbf{Prompt Formats}} & \head{0.6cm}{\textbf{Intent Acc}} & \head{0.5cm}{\textbf{Slot F1}} \\
\hline
 & Simple + Tag & \textbf{98.43} & 86.04 \\
ATIS & Simple + Extractive Sentinel & 97.76 & 93.12\\
 & Simple + Sentinel Tag & 98.21 & \textbf{94.26} \\
\hline
 & Simple + Tag & 97.85 & 89.11 \\
SNIPS & Simple + Extractive Sentinel & \textbf{98.71}  & 92.88 \\
& Simple + Sentinel Tag & 98.14 & \textbf{94.51} \\
\hline
 & Simple + Tag & 88.68 & 72.91 \\
 & Simple + Extractive Sentinel & 88.33 & 73.42 \\
 & Simple + Sentinel Tag & 87.51 & 75.36 \\
MASSIVE & Structured + Tag & \textbf{88.73} & 75.72 \\ 
 & Structured + Extractive Sentinel & 87.82 & 75.13 \\
 & Structured + Sentinel & 88.01 & \textbf{80.45} \\
\hline
\end{tabular}
\end{table}

\begin{table*}[t]
\centering
\small
\caption{Mitigation results of data augmentation and PPCL on MASSIVE dataset. We show results with different augmentation sizes and different loss functions. For multi-sample augmentation the training size increase by $\sim 50k$, for single sample it is similar to the original size.}
\label{tab:ablation}
\begin{tabular}{llclrrrr}
\hline
\textbf{Perturb} & \textbf{Mitigation} & \textbf{Augmentation} & \textbf{Loss} & \textbf{IC-PDR} & \textbf{Recovery} & \textbf{SF-PDR} & \textbf{Recovery} \\
\hline
 & Baseline & - & $\mathcal{L}_c$ & 16.67 & - & 40.75 & - \\
 & JS Loss & +3k & $\mathcal{L}_c+\mathcal{L}_{js}$ & 15.74 & 5\% & 32.80 & 19\%\\
Oronyms & Perturb Loss & +3k & $\mathcal{L}_c+\mathcal{L}_p$ & 8.95 & 46\% & 18.44 & 55\% \\
 & Perturb Loss & +50k & $\mathcal{L}_c+\mathcal{L}_p$ & 9.02 & 45\% & 19.73 & 51\% \\
 & PPCL (JS + Perturb Loss) & +3k & $\mathcal{L}_c+\mathcal{L}_p +\mathcal{L}_{js}$  & \textbf{8.74} & \textbf{47\%} & \textbf{15.41} & \textbf{62\%} \\
\hline
 & Baseline & - & $\mathcal{L}_c$ & 13.94 & - & 9.72 & - \\
 & JS Loss & +5k & $\mathcal{L}_c+\mathcal{L}_{js}$ & 12.11 & 13\% & 7.83 & 19\%\\
Synonyms & Perturb Loss & +5k & $\mathcal{L}_c+\mathcal{L}_p$ & 5.59 & 60\% & 5.13 & 47\% \\
 & Perturb Loss & +50k & $\mathcal{L}_c+\mathcal{L}_p$ & 4.01 & 71\% & 4.49 & 53\% \\ 
 & PPCL (JS + Perturb Loss) & +5k & $\mathcal{L}_c+\mathcal{L}_p +\mathcal{L}_{js}$ & \textbf{3.74} & \textbf{73\%} & \textbf{1.44} & \textbf{85\%} \\
\hline
 & Baseline & - & $\mathcal{L}_c$ & 8.62 & - & 16.14 & - \\
 & JS Loss & +6k & $\mathcal{L}_c+\mathcal{L}_{js}$ & 7.79 & 9\% & 15.10 & 6\% \\
Paraphrases & Perturb Loss & +6k & $\mathcal{L}_c+\mathcal{L}_p$ & 5.92 & 31\% & 8.89 & 45\% \\
 & Perturb Loss & +50k & $\mathcal{L}_c+\mathcal{L}_p$ & \textbf{3.69} & \textbf{57\%} & \textbf{4.24} & \textbf{74\%} \\
 & PPCL (JS + Perturb Loss) & +6k & $\mathcal{L}_c+\mathcal{L}_p+\mathcal{L}_{js}$ & \textbf{3.69} & \textbf{57\%} & 6.36 & 60\% \\
\hline
\end{tabular}
\end{table*}


\subsection{Performance drop due to Prompt Perturbations}
\noindent
Table \ref{tab:cases} illustrates examples of clean and perturbed utterances and their difference in model predictions even though the BertScores between the clean and perturbed samples are higher than 0.85. We show the relative performance drops resulting from the following three perturbations: oronyms, synonyms, and paraphrases, on MASSIVE dataset in Table \ref{tab:pdrs}. The results of ATIS and SNIPS are shown in Appendix. Results show that discriminative models, ICL approaches, and LLMs with instruction fine-tuning are vulnerable to these perturbations with large performance drops. Notably, the performance drops are more significant with oronym perturbations, particularly in SF tasks. 

These findings highlight the vulnerabilities of both discriminative and generative models when exposed to perturbed data, underscoring the importance of addressing robustness issues to ensure the reliability and effectiveness of these models in real-world applications. Identifying and mitigating the impact of perturbations, especially in tasks involving sequence labeling like SF, are critical problems to improve the performance and generalizability of these models.

\begin{table}[H]
\centering
\small
\caption{Comparison of model performance drops as a result of prompt perturbations, on MASSIVE dataset. The smaller PDR values imply higher model robustness.}
\label{tab:pdrs}
\begin{tabular}{llrr}
\hline
\textbf{Perturb} & \textbf{Model} & \textbf{IC-PDR} & \textbf{SF-PDR} \\
\hline
 & JointBERT & 21.53 & 47.47 \\
 & JointBERT+CRF & 20.45 & 47.41 \\
 & GPT3.5-ZS & 1.15 & - \\
Oronyms  & GPT3.5-FS & 30.55 & 35.05 \\
 & GPT2+SFT & 20.83 & 58.40 \\
 & LLaMA-7b+SFT & 16.67 & 40.75 \\
\hline
 & JointBERT & 13.42 & 7.49 \\
 & JointBERT+CRF & 13.21 & 7.31 \\
 & GPT3.5-ZS & 6.95 & - \\
Synonyms  & GPT3.5-FS & 16.71 & 8.3 \\
 & GPT2+SFT & 17.14 & 10.74 \\
 & LLaMA-7b+SFT & 13.94 & 9.72 \\
\hline
 & JointBERT & 7.09 & 13.45 \\
 & JointBERT+CRF & 8.82 & 15.19 \\
 & GPT3.5-ZS & 9.09 & - \\
Paraphrases  & GPT3.5-FS & 9.88 & 16.2 \\
 & GPT2+SFT & 7.13 & 17.63 \\
 & LLaMA-7b+SFT & 8.62 & 16.14 \\
\hline
\end{tabular}
\end{table}

\subsection{PPCL Mitigation Results}
\noindent
We share results from two mitigation approaches for improving robustness of LLMs against prompt perturbations: data augmentation and PPCL. We show results with different augmentation sizes and different combinations of loss functions on MASSIVE dataset are in Table \ref{tab:ablation}. All these are done on LLaMA-7b model. Both approaches recover significant performance drop. The ones where multiple perturbed samples are added for each clean sample the training data size increases by 50k or more. For example, data augmentation with one perturbed sample per clean sample, along with perturbation loss, shown as $\mathcal{L}_C + \mathcal{L}_P$ recovers performance drops up to 45\% on IC and 51\% on SF tasks, respectively for Oronym perturbation. When augmented with 5 perturbed samples per clean sample, it performs better. However, PPCL, with only 1 perturbed sample per clean, which include perturbation loss and JS loss, outperforms multiple sample augmentation in all cases, except for SF in paraphrase perturbation. For paraphrase perturbation, PPCL recovers 60\% of SF-PDR compared to 74\% by multi-sample augmentation, but at one-tenth the augmentation size. On an average, PPCL is able to recover 59\% in IC and 69\% in SF performance drops. In comparison, multi-sample augmentation is able to recover 58\% in IC and 59\% in SF. PPCL achieves the recoveries with one-tenth the augmentation size. PPCL comparisons with augmentation on ATIS and SNIPS datasets as shown in Appendix, indicating the generalizability and effectiveness of our approach across different domains and datasets.

\subsection{Ablation Studies}
\noindent
In our training objective, there are three different terms in Eq. \ref{eq:objective}, and to better understand their contributions towards improving the robustness of LLMs against perturbations, we conducted an ablation study as shown in Table \ref{tab:ablation}. 

From the experimental findings, it is evident that the models achieve the best performance when all three loss terms ($\mathcal{L}_c,\ \mathcal{L}_p, \ \mathcal{L}_{js}$) in the training objective are utilized. This indicates that each of these terms plays a significant role in enhancing the robustness of the models. PPCL outperforms multi-sample augmentation with a fraction of augmentation volume in 5 out of 6 tasks in Massive data. 

\subsection{Failure and Saved Examples}
We provide two case studies in Table \ref{tab:cases} to illustrate some failure responses due to the perturbations and the recoveries of these failures applying our proposed perturbation consistency learning. In these two examples, we can observe that oronym substitution and paraphrasing lead the model to generate incorrect responses. These incorrect responses (red lines) are characterized as failure cases, as they do not accurately capture the user's intents or the relevant information in the utterances. However, after re-training the model with our perturbation consistency learning approach, we can see improvement. The model is now able to generate the correct responses, which are demonstrated in blue lines. 


\begin{table*}[t]
\centering
\small
\caption{Some examples of clean and perturbed utterances, with BertScore $>$ 0.85. Red lines are a result of perturbation. Blue lines are post PPCL mitigation.}
\label{tab:cases}
\begin{tabular}{lllll}
\hline
Perturbations & Utterances                          & Pred\_Domain & Pred\_Intent        & Pred\_Slots                          \\ \hline
Clean      & create an alarm for today at ten am & alarm        & alarm\_set          & {[}today: date , ten am: time{]} \\
\textcolor{red}{Paraphrase}    & \textcolor{red}{set a reminder for today at ten am}  & \textcolor{red}{calendar}     & \textcolor{red}{calendar\_set}       & \textcolor{red}{{[}today: date , ten am: time{]}} \\ 
\textcolor{blue}{Paraphrase}    & \textcolor{blue}{set a reminder for today at ten am}  & \textcolor{blue}{alarm}        & \textcolor{blue}{alarm\_set}          & \textcolor{blue}{{[}today: date , ten am: time{]}}   \\ \hline
Clean      & give   me more lite                 & iot          & iot\_hue\_lightup   & {[}{]}  \\ 
\textcolor{red}{Oronym}        & \textcolor{red}{give mi moore lite}              & \textcolor{red}{email}        & \textcolor{red}{email\_querycontact} & \textcolor{red}{{[}mi moore: person{]}} \\ 
\textcolor{blue}{Oronym}        & \textcolor{blue}{give mi moore lite}                  & \textcolor{blue}{iot}          & \textcolor{blue}{iot\_hue\_lightup}   & \textcolor{blue}{{[}{]}}     \\ \hline
\end{tabular}
\end{table*}


